ADVISER: AI-Driven Vaccination Intervention Optimiser for Increasing Vaccine Uptake in Nigeria

More than 5 million children under five years die from largely preventable or treatable medical conditions every year, with an overwhelmingly large proportion of deaths occurring in under-developed countries with low vaccination uptake. One of the United Nations' sustainable development goals (SDG 3) aims to end preventable deaths of newborns and children under five years of age. We focus on Nigeria, where the rate of infant mortality is appalling. We collaborate with HelpMum, a large non-profit organization in Nigeria to design and optimize the allocation of heterogeneous health interventions under uncertainty to increase vaccination uptake, the first such collaboration in Nigeria. Our framework, ADVISER: AI-Driven Vaccination Intervention Optimiser, is based on an integer linear program that seeks to maximize the cumulative probability of successful vaccination. Our optimization formulation is intractable in practice. We present a heuristic approach that enables us to solve the problem for real-world use-cases. We also present theoretical bounds for the heuristic method. Finally, we show that the proposed approach outperforms baseline methods in terms of vaccination uptake through experimental evaluation. HelpMum is currently planning a pilot program based on our approach to be deployed in the largest city of Nigeria, which would be the first deployment of an AI-driven vaccination uptake program in the country and hopefully, pave the way for other data-driven programs to improve health outcomes in Nigeria.

==> causalDiagram.tex <==
\begin{figure}
\centering
\begin{tikzpicture} 
\coordinate (O) at (0,0);
\node[basicNode] (X) {$X$}; 
\node (Z) [basicNode, above of=X, xshift=1.5cm, yshift=0.5cm, align=center] {$Z$};
\node (Y) [basicNode, right of=X, xshift=2cm, align=center] {$Y$};
\node (UX) [transNode, above of=X] {$U_X$};
\node (UY) [transNode, above of=Y] {$U_Y$};
\node (UZ) [transNode, above of=Z] {$U_Z$};
\draw[->] (X) -- (Y);
\draw[->] (Z) -- (Y);
\draw[->] (0,0.85) -- (X);
\draw[->] (3,0.85) -- (Y);
\draw[->] (1.5,2.35) -- (Z);
\end{tikzpicture}
\caption{Computing the impact of making phone calls to mothers}
\label{fig:causal}
\end{figure}

==> final_formulation.tex <==
\noindent \textbf{Constraints}:
\begin{enumerate}
    \item Eligibility Constraint: Each mother must be eligible for the vaccine when she is being targeted for an intervention. 
    \[y_{itj} \leq a(i, t) \;\;\; \forall i \in M, t \in T, j \in I \setminus v.\]
    \[z_{itc} \leq a(i,t) \;\;\; \forall i \in M, t \in T, c \in C.
    \]
    \item Vaccine Drive Constraint: If a mother is being targeted for a vaccination drive at a given location and time, there must exist such a drive.
    \[z_{itc} \leq x_{tc} \;\;\; \forall i \in M, t \in T, c \in C\]
    \item Location Constraint: Only mothers that live within a certain distance of a drive can be targeted for the drive.
    \[z_{itc} \, d_{ic} \leq r \;\;\; \forall i \in M, t \in T, c \in C\]
    \item Budget Constraint: The total monetary budget of the organization cannot be exceeded.
    \[\sum_{ i \in M} \sum_{t \in T} \sum_{I \in I \setminus V} y_{itj} q_i + \sum_{t \in T} \sum_{c \in C} x_{tc} q_v \leq b\]
    \item At most one intervention constraint: Each mother can be targeted for at most one intervention.
    \[
    \sum_{t \in T} \sum_{j \in I \setminus v} y_{itj} + \sum_{t \in T} \sum_{c \in C} z_{itc} \leq 1 \;\;\;\; \forall i \in  M
    \]
\end{enumerate}
\noindent \textbf{VRP Constraints}:
\begin{enumerate}
    \item 
\end{enumerate}


\noindent \textbf{Objective}:

\[
x^{*},y^{*},z^{*} = \argmax_{x,y,z} \sum_{i \in M} \sum_{t \in T} \sum_{j \in I \setminus v} y_{itj} p_{ij} + \sum_{ i \in M} \sum_{t \in T} \sum_{c \in C} z_{itc}p_{iv}
\]
\noindent \textbf{Revised Objective}:

\[
x^{*},y^{*},z^{*} = \argmax_{x,y,z} \sum_{i \in M} \sum_{t \in T} \sum_{j \in I \setminus v} y_{itj} p_{ij} + \sum_{ i \in M} \sum_{t \in T} \sum_{c \in C} z_{itc}p_{iv}
\]

==> gen_graphs.tex <==


% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Objective values (D1),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 13354.28) (7.2, 13548.07) (7.4, 13745.84) (7.6, 13932.04)
%     (7.8, 14110.16) (8, 14287.23) (8.2, 14459.03) (8.4, 14637.21)
%     (8.6, 14637.21)};
% \addplot
% 	coordinates {
%     (7, 28139.13) (7.2, 28647.83) (7.4, 28254.08) (7.6, 28661.92)
%     (7.8, 29462.08) (8, 29381.25) (8.2, 29812.69) (8.4, 30198.89)
%     (8.6, 30198.89)};
% \addplot
% 	coordinates {
%     (7, 39819.07) (7.2, 39837.43) (7.4, 39852.05) (7.6, 39863.48)
%     (7.8, 39872.68) (8, 39880.05) (8.2, 39886.05) (8.4, 39890.66)
%     (8.6, 39890.66)};
% % % \legend{RWB, HILP, ADVISER-NV}
% \end{axis}
% \end{tikzpicture}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Objective values (D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 13354.28) (7.2, 13548.07) (7.4, 13745.84) (7.6, 13932.04)
%     (7.8, 14110.16) (8, 14287.23) (8.2, 14459.03) (8.4, 14637.21)
%     (8.6, 14637.21)};
% \addplot
% 	coordinates {
%     (7, 28139.13) (7.2, 28647.83) (7.4, 28254.08) (7.6, 28661.92)
%     (7.8, 29462.08) (8, 29381.25) (8.2, 29812.69) (8.4, 30198.89)
%     (8.6, 30198.89)};
% \addplot
% 	coordinates {
%     (7, 39237.1171) (7.2, 39351.17) (7.4, 39441.97) (7.6, 39502.85)
%     (7.8, 39543.88) (8, 39573.95) (8.2, 39597.92) (8.4, 39617.23)
%     (8.6, 39617.23)};
% % % % \legend{RWB, HILP, ADVISER-NV}
% \end{axis}
% \end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=No allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 21166) (7.2, 20666) (7.4, 20166) (7.6, 19666)
%     (7.8, 19166) (8, 18666) (8.2, 18166) (8.4, 17666)
%     (8.6, 17166)};
% \addplot
% 	coordinates {
%     (7, 13193) (7.2, 12578) (7.4, 13017) (7.6, 12570)
%     (7.8, 11623) (8, 11708) (8.2, 11213) (8.4, 10785)
%     (8.6, 10785)};
% \addplot
% 	coordinates {
%     (7, 1747) (7.2, 1513.5) (7.4, 1285.5) (7.6, 1068)
%     (7.8, 893.5) (8, 763) (8.2, 636) (8.4, 505.5)
%     (8.6, 505.5)};
% % % \legend{RWB, HILP, ADVISER-NV}
% \end{axis}
% \end{tikzpicture}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%% OBJECTIVE VALUE GRAPHS %%%%%%%%%%%%
% \begin{tikzpicture}
% \begin{axis}[
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	major x tick style = transparent,
% 	ylabel=Objective values (D1),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$), 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 27467.34) (7.2, 27584.8) (7.4, 27699.04) (7.6, 27821.3)
%     (7.8, 27940.15) (8, 28058.75) (8.2, 28183.38) (8.4, 28301.54)
%     (8.6, 28301.54)};
% \addplot
% 	coordinates {
%     (7, 33955.31) (7.2, 33983.59) (7.4, 34444.41) (7.6, 34712.21)
%     (7.8, 34718.53) (8, 35036.16) (8.2, 35238.89) (8.4, 35508.94)
%     (8.6, 35508.94)};
% \addplot
% 	coordinates {
%     (7, 39910.25) (7.2, 39938.89) (7.4, 39955.97) (7.6, 39966.71)
%     (7.8, 39973.95) (8, 39977.13) (8.2, 39978.66) (8.4, 39979.22)
%     (8.6, 39979.22)};
% % \legend{}
% % \legend{RWB, HILP, ADVISER}
% \end{axis}
% \end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{tikzpicture}
% \begin{axis}[
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	major x tick style = transparent,
% 	ylabel=Objective values (D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$), 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 13354.28) (7.2, 13548.07) (7.4, 13745.84) (7.6, 13932.04)
%     (7.8, 14110.16) (8, 14287.23) (8.2, 14459.03) (8.4, 14637.21)
%     (8.6, 14637.21)};
% \addplot
% 	coordinates {
%     (7, 28139.13) (7.2, 28647.83) (7.4, 28254.08) (7.6, 28661.92)
%     (7.8, 29462.08) (8, 29381.25) (8.2, 29812.69) (8.4, 30198.89)
%     (8.6, 30198.89)};
% \addplot
% 	coordinates {
%     (7, 39421.58) (7.2, 39548.59) (7.4, 39663.02) (7.6, 39751.22)
%     (7.8, 39808.48) (8, 39842.62) (8.2, 39862.42) (8.4, 39873.09)
%     (8.6, 39873.09)};
% % \legend{RWB, HILP, ADVISER}
% \end{axis}
% \end{tikzpicture}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%% NO ALLOCATION GRAPH COMBINED %%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=No allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$), 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 21162) (7.2, 20662) (7.4, 20162) (7.6, 19662)
%     (7.8, 19162) (8, 18662) (8.2, 18162) (8.4, 17662)
%     (8.6, 17162)
%     };
% \addplot
% 	coordinates {
%     (7, 13065) (7.2, 12689.5) (7.4, 12413) (7.6, 11906)
%     (7.8, 11442.5) (8, 11145) (8.2, 10681) (8.4, 10183)
%     (8.6, 10183)
%     };
% \addplot
% 	coordinates {
%     (7, 914) (7.2, 661) (7.4, 484) (7.6, 284)
%     (7.8, 154) (8, 82) (8.2, 33) (8.4, 11.5)
%     (8.6, 11.5)
%     };
% % \legend{RWB, HILP, ADVISER}
% \end{axis}
% \end{tikzpicture}


% Mention ADVISER NV in the caption 
% \begin{tikzpicture}
%     \begin{axis}[
%         major x tick style = transparent,
%         % ybar=2*\pgflinewidth,
%         ylabel = {Intervention Allocations (D1 + D2)},
%         symbolic x coords={Drive, Bus, Voucher, Phone, None, None2},
%         % xtick = data,
%         % enlarge x limits=0.25,
%         x tick label style={
% 		/pgf/number format/1000 sep=},
%     	enlargelimits=0.05,
%     	legend style={at={(0.5,-0.1)},
%     	anchor=north,legend columns=-1},
%     	ybar interval=0.7,
%     ]
%     \addplot
%     coordinates {(Drive, 7368.5) (Bus, 608) (Voucher, 1114.5) (Phone, 11497) (None, 19412) (None2, 19412) };
%     \addplot
%     coordinates {(Drive, 27932.25) (Bus, 0) (Voucher, 167.36) (Phone, 327.03) (None, 11573.37) (None2, 11573.37)};
%     \addplot
%     coordinates {(Drive, 29902.32) (Bus, 332.15) (Voucher, 742.29) (Phone, 2721.39) (None, 6301.85) (None2, 6301.85)};
%     % \legend{RWB, HILP, ADVISER-NV}
%     \end{axis}
% \end{tikzpicture}

% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Drive allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 7368.5) (7.2, 7368.5) (7.4, 7368.5) (7.6, 7368.5)
%     (7.8, 7368.5) (8, 7368.5) (8.2, 7368.5) (8.4, 7368.5)
%     (8.6, 7368.5)};
% \addplot
% 	coordinates {
%     (7, 26443.5) (7.2, 26840) (7.4, 27105.5) (7.6, 27599)
%     (7.8, 28060.5) (8, 28342) (8.2, 28799) (8.4, 29333.5)
%     (8.6, 29333.5)};
% \addplot
% 	coordinates {
%     (7, 36569) (7.2, 36569) (7.4, 36569) (7.6, 36569)
%     (7.8, 36569) (8, 36569) (8.2, 36569) (8.4, 36569)
%     (8.6, 36569)};
% % \legend{RWB, HILP, ADVISER-NV}
% \end{axis}
% \end{tikzpicture}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Vehicle route allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 608) (7.2, 608) (7.4, 608) (7.6, 608)
%     (7.8, 608) (8, 608) (8.2, 608) (8.4, 608)
%     (8.6, 608)};
% \addplot
% 	coordinates {
%     (7, 0) (7.2, 0) (7.4, 0) (7.6, 0)
%     (7.8, 0) (8, 0) (8.2, 0) (8.4, 0)
%     (8.6, 0)};
% \addplot
% 	coordinates {
%     (7, 362) (7.2, 416) (7.4, 495.5) (7.6, 525.5)
%     (7.8, 577) (8, 654) (8.2, 694) (8.4, 729)
%     (8.6, 729)};
% % % % \legend{RWB, HILP, ADVISER-NV}
% \end{axis}
% \end{tikzpicture}

% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Voucher allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 1114.5) (7.2, 1114.5) (7.4, 1114.5) (7.6, 1114.5)
%     (7.8, 1114.5) (8, 1114.5) (8.2, 1114.5) (8.4, 1114.5)
%     (8.6, 1114.5)};
% \addplot
% 	coordinates {
%     (7, 141) (7.2, 156.5) (7.4, 156.5) (7.6, 170)
%     (7.8, 169.5) (8, 172.5) (8.2, 182.5) (8.4, 176)
%     (8.6, 176)};
% \addplot
% 	coordinates {
%     (7, 316) (7.2, 427.5) (7.4, 542.5) (7.6, 678.5)
%     (7.8, 836.5) (8, 962.5) (8.2, 1127) (8.4, 1301.5)
%     (8.6, 1301.5)};
% % % % \legend{RWB, HILP, ADVISER-NV}
% \end{axis}
% \end{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Phone allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 9747) (7.2, 10247) (7.4, 10747) (7.6, 11247)
%     (7.8, 11747) (8, 12247) (8.2, 12747) (8.4, 13247)
%     (8.6, 13247)};
% \addplot
% 	coordinates {
%     (7, 350.5) (7.2, 314) (7.4, 325) (7.6, 325)
%     (7.8, 327.5) (8, 340.5) (8.2, 337.5) (8.4, 307.5)
%     (8.6, 307.5)};
% \addplot
% 	coordinates {
%     (7, 1006) (7.2, 1074) (7.4, 1107.5) (7.6, 1159)
%     (7.8, 1124) (8, 1051.5) (8.2, 974) (8.4, 895)
%     (8.6, 1135)};
% % % % \legend{RWB, HILP, ADVISER-NV}
% \end{axis}
% \end{tikzpicture}


% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Drive allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 7368.5) (7.2, 7368.5) (7.4, 7368.5) (7.6, 7368.5)
%     (7.8, 7368.5) (8, 7368.5) (8.2, 7368.5) (8.4, 7368.5)
%     (8.6, 7368.5)};
% \addplot
% 	coordinates {
%     (7, 26443.5) (7.2, 26840) (7.4, 27105.5) (7.6, 27599)
%     (7.8, 28060.5) (8, 28342) (8.2, 28799) (8.4, 29333.5)
%     (8.6, 29333.5)};
% \addplot
% 	coordinates {
%     (7, 38557.5) (7.2, 38721) (7.4, 38846) (7.6, 39069.5)
%     (7.8, 39219) (8, 39351) (8.2, 39455) (8.4, 39539)
%     (8.6, 39539)};
% % \legend{RWB, HILP, ADVISER}
% \end{axis}
% \end{tikzpicture}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Vehicle route allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 608) (7.2, 608) (7.4, 608) (7.6, 608)
%     (7.8, 608) (8, 608) (8.2, 608) (8.4, 608)
%     (8.6, 608)};
% \addplot
% 	coordinates {
%     (7, 0) (7.2, 0) (7.4, 0) (7.6, 0)
%     (7.8, 0) (8, 0) (8.2, 0) (8.4, 0)
%     (8.6, 0)};
% \addplot
% 	coordinates {
%     (7, 15) (7.2, 27) (7.4, 87.5) (7.6, 54.5)
%     (7.8, 85) (8, 61.5) (8.2, 21.5) (8.4, 7.5)
%     (8.6, 7.5)};
% % % % \legend{RWB, HILP, ADVISER}
% \end{axis}
% \end{tikzpicture}

% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Voucher allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 1114.5) (7.2, 1114.5) (7.4, 1114.5) (7.6, 1114.5)
%     (7.8, 1114.5) (8, 1114.5) (8.2, 1114.5) (8.4, 1114.5)
%     (8.6, 1114.5)};
% \addplot
% 	coordinates {
%     (7, 141) (7.2, 156.5) (7.4, 156.5) (7.6, 170)
%     (7.8, 169.5) (8, 172.5) (8.2, 182.5) (8.4, 176)
%     (8.6, 176)};
% \addplot
% 	coordinates {
%     (7, 113.5) (7.2, 190.5) (7.4, 242) (7.6, 304.5)
%     (7.8, 329.5) (8, 371.5) (8.2, 419.5) (8.4, 407.5)
%     (8.6, 407.5)};
% % % % \legend{RWB, HILP, ADVISER}
% \end{axis}
% \end{tikzpicture}

% \begin{tikzpicture}
% \begin{axis}[
%     major x tick style = transparent,
% 	x tick label style={
% 		/pgf/number format/1000 sep=},
% 	ylabel=Avg. Phone allocations (D1 + D2),
% 	enlargelimits=0.05,
% 	xlabel=Budget ($\times \$10^3$),
% 	legend style={at={(0.5,-0.2)},
% 	anchor=north,legend columns=-1},
% 	ybar interval=0.7,
% ]
% \addplot
% 	coordinates {
%     (7, 9747) (7.2, 10247) (7.4, 10747) (7.6, 11247)
%     (7.8, 11747) (8, 12247) (8.2, 12747) (8.4, 13247)
%     (8.6, 13247)};
% \addplot
% 	coordinates {
%     (7, 350.5) (7.2, 314) (7.4, 325) (7.6, 325)
%     (7.8, 327.5) (8, 340.5) (8.2, 337.5) (8.4, 307.5)
%     (8.6, 307.5)};
% \addplot
% 	coordinates {
%     (7, 400) (7.2, 400.5) (7.4, 340.5) (7.6, 287.5)
%     (7.8, 212.5) (8, 134.5) (8.2, 71) (8.4, 34.5)
%     (8.6, 34.5)};
% % % % \legend{RWB, HILP, ADVISER}
% \end{axis}
% \end{tikzpicture}


==> macro.tex <==

\usepackage{verbatim}


\newtheorem{proposition}{Proposition}
\newthoerem{theorem}{theorem}
\newcommand{\toref}{\textcolor{red}{REF}}




==> tables/runtime.tex <==
% \begin{table}
% \caption{Average runtime of algorithms in seconds}
% \centering
% \begin{tabularx}{0.47\textwidth}{
%   | >{\centering\arraybackslash}X 
%   | >{\centering\arraybackslash}X | }
% \hline
%  Method   & Average-Time (seconds) \\
% \hline
%  ADVISER  & 254 \\
%  HILP     & 4387 \\
% \hline
% \end{tabularx}
% \label{tab:time}
% \end{table}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
Method  & Average Computation Time (in sec) \\ \midrule
ADVISER & 254                               \\
HILP    & 4387                              \\
RWB     & 8                                 \\ \bottomrule
\end{tabular}
\caption{Computation time for the proposed approaches. The computation time does not consider the routing solver. Routes are generated separately and are provided as input to each algorithm.}
\label{tab:time}
\end{table}
